Hairmony: Fairness-aware hairstyle classification

We present a method for prediction of a person's hairstyle from a single image. Despite growing use cases in user digitization and enrollment for virtual experiences, available methods are limited, particularly in the range of hairstyles they can capture. Human hair is extremely diverse and lacks any universally accepted description or categorization, making this a challenging task. Most current methods rely on parametric models of hair at a strand level. These approaches, while very promising, are not yet able to represent short, frizzy, coily hair and gathered hairstyles. We instead choose a classification approach which can represent the diversity of hairstyles required for a truly robust and inclusive system. Previous classification approaches have been restricted by poorly labeled data that lacks diversity, imposing constraints on the usefulness of any resulting enrollment system. We use only synthetic data to train our models. This allows for explicit control of diversity of hairstyle attributes, hair colors, facial appearance, poses, environments and other parameters. It also produces noise-free ground-truth labels. We introduce a novel hairstyle taxonomy developed in collaboration with a diverse group of domain experts which we use to balance our training data, supervise our model, and directly measure fairness. We annotate our synthetic training data and a real evaluation dataset using this taxonomy and release both to enable comparison of future hairstyle prediction approaches. We employ an architecture based on a pre-trained feature extraction network in order to improve generalization of our method to real data and predict taxonomy attributes as an auxiliary task to improve accuracy. Results show our method to be significantly more robust for challenging hairstyles than recent parametric approaches.

==> tables/ablation_qual.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{tabular}{p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}p{1.41cm}}
    % \setlength{\tabcolsep}{0.1\linewidth}
         Input & \textbf{Ours} & ResNet50 & ResNet101 & Prediction choice & Input & \textbf{Ours} & ResNet50 & ResNet101 & Prediction choice \\
    \end{tabular}
    \includegraphics[width=\linewidth]{figures/comparison_image_faves_combined_divide_ours.png}
    \caption{Qualitative results corresponding to our best model, ResNet-50, and ResNet-101 (Table 5 of the main paper). We report Top-3 predictions for all models.}
    \label{fig:comparison}
\end{figure*}
